Joining Entities Across Relation and Graph with a Unified Model

This paper introduces RG (Relational Genetic) model, a revised relational model to represent graph-structured data in RDBMS while preserving its topology, for efficiently and effectively extracting data in different formats from disparate sources. Along with: (a) SQL$_\delta$, an SQL dialect augmented with graph pattern queries and tuple-vertex joins, such that one can extract graph properties via graph pattern matching, and "semantically" match entities across relations and graphs; (b) a logical representation of graphs in RDBMS, which introduces an exploration operator for efficient pattern querying, supports also browsing and updating graph-structured data; and (c) a strategy to uniformly evaluate SQL, pattern and hybrid queries that join tuples and vertices, all inside an RDBMS by leveraging its optimizer without performance degradation on switching different execution engines. A lightweight system, WhiteDB, is developed as an implementation to evaluate the benefits it can actually bring on real-life data. We empirically verified that the RG model enables the graph pattern queries to be answered as efficiently as in native graph engines; can consider the access on graph and relation in any order for optimal plan; and supports effective data enrichment.

==> sec-example.tex <==
\stitle{Importance of pattern matching}. Graph pattern matching has been considered as one of the core functionalities for querying graphs~\cite{barcel2011querying, barcel2013querying, davoudian2018survey, peter2012query, angles2017foundations, angles2018GCORE, angles2012comparison, angles2018property, hogan2021knowledge, alin2022Graph},
which is enabled as a feature in most of the graph query languages~\cite{sparql, sparql11, TinkerPop, francis2018cypher, pienta2016VISAGE, huahai2008graphs,rest2016PGQL,ma2016g,TigerGraph,openCypher},
and is supported by numerous 
GDBMS~\cite{allegrogaph, DEX, Filament, GStore, Infinitegraph, SonesGraphDB, vertexdb, neo4j, iordanov2010HyperGraphDB, TinkerPop, TigerGraph}.
Pattern queries  are becoming increasing ubiquitous:
$16/60$ of literatures in~\cite{hegeman2018survey},
$32/40$ of practitioners in~\cite{angles2018GCORE},
$14/36$ of researchers and
$19/53$ of practitioners in~\cite{SahuMSLO2020ubiquity}
concentrate on graph pattern matching.
They are also adopted in a wide-range of real world applications,
across biology~\cite{koyuturk2004efficient, li2005interaction, royer2008unraveling},
security~\cite{jiang2010identifying}, 
software engineering~\cite{cheng2009identifying, eichinger2008mining, liu2006gplag, maxwell2010diagnosing, surian2010mining, zimmermann2008predicting}, chemistry~\cite{nijssen2004frequent, wegner2006data} and others~\cite{FraudDetect}.
The polyglot system developed here would 
therefore consider the SQL and pattern matching as 
the semantics for the query on relational data and graph data respectively.


\stitle{Application scenario of semantic joins}.
Consider a logistic company that maintains (1) 
a road network where the vertices
represent POIs, warehouses, transfer stations etc., and its
edges are labeled with distance; and
(2) relations to keep the profiles of customers
and their delivery orders. Each order should include 
the addresses of source and destination locations
provided by the user, which
are commonly diversified for the same location
and sometimes even inaccurate or incomplete.

With pattern matching
queries and semantic joins, especially mapping the addresses
to the vertices in the graph, the logistic company can 
achieve the following.

\sstab
(a) Find whether there is an appropriate 
transportation route (with bounded distance)
to deliver a set of orders in a single journey.

\sstab
(b) Recommend some collection points to the customer
regarding his order, which should be convenient
in terms of the distance and working hours.

\sstab
(c) Enrich/fix the attributes of customers and orders,
\eg zip code, by taking those from the road network.

\stitle{Comparing with previous works}.
As a \emph{``hot research topic in recent years''}~\cite{kiehn2022polyglot}, numerous approaches are 
in place to %allow user 
query across graph and relational data. 
However, according to the taxonomy from~\cite{tan2017enabling}, most of them are relation-based polyglot systems~\cite{zhao2017all, zhao2017graph, dave2016graphframes, jindal2014vertexica, jindal2015graph, fan2015case, quamar2016nscalespark, steer2017cytosm, xirogiannopoulos2017graphgen, da2020kaskade}.
Basically they only provide different mechanisms as \emph{``middleware''}~\cite{zhang2018unified,vilacca2013effective,rith2014speaking} for the graph query to be executed on the
relational engine, RDBMS or other engines with relational interface~\cite{zaharia2012resilient, armbrust2015spark}.
Meanwhile, although without a language-level extension to support hybrid query explicitly,
previous works also provided various relational solutions for graph data processing~\cite{sakr2009graphrel, jin2021making, abadi2007scalable, hassan2017empowering, sun2015sqlgraph, wilkinson2003efficient, matono2005path, schatzle2015s2rdf, mhedhbi2021a+}, especially for RDF data~\cite{mahmoudinasab2010experimental, ozsu2016survey, faye2012survey, kaoudi2015rdf, wylot2018rdf, modoni2014survey, sahoo2009survey, sakr2010relational, michel2014survey, abdelaziz2017survey, pan2018survey}. 
They are also considered as relation-graph polyglot system here since they can be easily extended with any work of graph-relation query mapping~\cite{sun2015sqlgraph, blakeley2006ado, o2008object, bergmann2012applying, steer2017cytosm, vidal2017computing, xirogiannopoulos2017graphgen, boncz2018g}.
However, although some of them try to optimize the RDBMS for more efficient graph data processing,
they are all less aggressive 
without touching the data organization
and therefore the performance improvement brought by the graph structure~\cite{guting1994graphdb, angles2008survey, cheng2019category, pacaci2017we, kolomivcenko2013analysis, mccoll2014performance, barmpis2014evaluation} cannot be expected to be fully obtained.

Meanwhile, principally speaking, the poly-store/multi-store~\cite{tan2017enabling,duggan2015bigdawg, kolev2016cloudmdsql, abouzeid2009hadoopdb} systems can take an advantage from different storage structure for different kinds of queries, although there %are actually 
does not exist such a system that can support graph data.
Previous works also extract information from relational data in various ways~\cite{da2020kaskade, hassan2018grfusion, hassan2017empowering, xirogiannopoulos2015graphgen, xirogiannopoulos2017graphgen, xirogiannopoulos2017extracting} to accelerate the graph query.
However, although it can be regarded as an advantage for this kind of systems to access across heterogeneous data store and execution engine~\cite{tan2017enabling, gupta2016cross}, 
it would still inevitability bring overhead that can be 
eliminated at the very beginning if there are a homogeneous representation for both sides of data.

The \emph{incompatibility} between the relational model and the graph model the previous
systems deploy prevents an \emph{in-depth} fusion of the hybrid query from being considered.
This would bring overhead for cross model access.
Taking the GRFusion~\cite{hassan2018grfusion, hassan2017empowering}, 
the closest one to the polyglot system proposed here,
%that allows users to query across the relational and graph data, 
as an example to demonstrate what actual limitation are brought by the \emph{incompatible} models.
In GRFusion,
only restricted accesses are allowed on graph data and
they can only be supported by the coarse-grained physical operators.
The planning space for the hybrid queries is therefore relatively limited and fail to provide a comprehensive optimization,
which also prevents complicated query on graph side to be executed efficiently.


In spite of the difference in format, the \emph{variety} of big data~\cite{russom2011big, sagiroglu2013big, buhl2013big, laney20013d} also requires the practitioners to analyze data from diverse sources~\cite{uselton1998multi}, which therefore requires the semantic connection among the data to be considered~\cite{christophides2020overview, fan2022linking}. 
Meanwhile, the structure of graph can also be messy for the users to obtain the information they need,
\ie it can be hard for the users to write the correct pattern to query the information they need, even only
using a path~\cite{francis2018cypher, hassan2018grfusion, hassan2017empowering}.

%A simply taxonomy is made here  to distinguish different kinds of hybrid query: 
% with/without knowing vertex-tuple matching; 
% with/without structured data extracted from graph.

The above two problems can be addressed with two well-studied approaches: (heterogeneous) entity resolution~\cite{christophides2020overview, papadakis2020blocking, naumann2010introduction, bellahsene2011evaluating, getoor2012entity, binette2022almost, fan2022linking}, to capture the semantic \emph{vertex-tuple} connection; 
and graph schema extraction~\cite{wang2000approximate, anutariya2018vizlod, frozza2020approach, zouaq2020schema, nestorov1998extracting, kellou2022survey, vcebiric2019summarizing, wu2008identifying, spahiu2016abstat}, to obtain structured data for querying.


In this work, a mild extension of SQL, similar to the ones in ~\cite{ma2016g, zhao2019sql, andries1996hybrid, hassan2018grfusion, hassan2017empowering}, is provided with 
corresponding query rewriting strategy. The extension is more convenient to be further extended to consider the semantic connection, compared to previous works.
Meanwhile,
different from previous works for schema extraction, 
our method allows the structuralized information to be extracted as \emph{view}~\cite{stonebraker1975implementation}. This avoids the overhead for materializing the extracted data.



==> sec-hybrid.tex <==
\vspace{-0.3ex}
%%%%%%%% Section 1 %%%%%%%%

\section{Hybrid Query Evaluation}
\label{sec-hybrid-query-evaluation}

\eat{
	Although graph pattern matching itself can be described equivalently with the relational algebra~\cite{jachiet2020optimization, bancilhon1989amateurs, agrawal1988alpha, abiteboul1995foundations, melton2001sql, nguyen2015join, sun2015sqlgraph, blakeley2006ado, o2008object, bergmann2012applying, steer2017cytosm, vidal2017computing, xirogiannopoulos2017graphgen, boncz2018g, jindal2014graphiql},
	it does not mean the optimal way for processing can thus be provided.
	
	The previous section shows how the proposed \ModelName model can uniformly represent both the relational and graph data and thus eliminate the cross-model access.
	It would be further demonstrated in this section how the hybrid query across relational and graph data can be evaluated with a larger unified plan space and seamless execution process.
}

It is stated previously that the unified representation of the relational and graph data can eliminate the cross-model access for a more efficient hybrid query.
It would be demonstrated in this section how the operators introduced in \ModelName model allow
the hybrid query plan to be also represented in a larger unified plan space for optimization and then be executed seamlessly.


\subsection{Operators Introduced in \ModelName Model}
\label{subsec-RX-model-operator}

In addition to introducing the pointer to conventional relational model, \ModelName model also brings more logical and physical operators in the query plan to explore through those pointers.
It then allows most of the optimization methods in native graph-based algorithms~\cite{huang2014query, cordella2004sub, han2019efficient, han2013turboiso, bhattarai2019ceci, bouhenni2021survey, yang2021huge} to be considered equivalently or even be directly plugged in here.
Meanwhile, the well-developed optimization and execution procedures for RDBMS can also be entirely inherited to optimize hybrid \ModelName query plan with minor modifications, which would be demonstrated in Section~\ref{subsec-query-graph} and Section \ref{subsec-hybrid-query-execution} respectively.

\eat{
\textcolor{red}{(A definition of the introduced operators?)
	Figure~\ref{fig-operator} demonstrates a typical exploration process of the operators introduced in \ModelName model. 
	Providing a \ModelName relation with a field of pointer, the exploration join can be performed as:
	(1) the ;
	(2) .
}
}

Since different tuples are connected by the introduced logic-level pointers, the exploration through them would thus be regarded as a kind of join operator, named as \textbf{exploration join} here.
Denoted as $R_b \; \vec{\bowtie}^{ \; p} [R_p]$, it means for each tuple $t_0 \in R_b$, iterate over all tuples pointed by the pointer in field $p$ of it, i.e. to find all $t_1 \in \psi_L(t_0.p)$, where the set of tuples $\psi_L(t_0.p)$ would be regarded as a subset of a virtual table $[R_p]$.
Different from the conventional relational join that can be evaluated from the relations on both sides, 
the exploration join can only be explored through the pointers from one direction, which bring more restrictions while some strategies would be introduced in Section~\ref{subsec-query-graph} to guarantee the generated query plan to be legal.
	
Meanwhile, another kind of join condition is also allowed to be considered by the pointer introduced here, named as \textbf{exploration join condition} which is denoted as $R_a \; \bowtie_{\; \psi_L(p).a \;  \ni \; b} R_b$.
It means for each tuple $t_a \in R_a$ and $t_b \in R_b$, join them together if there are at least one tuple $t_p \in \psi_L(t_a.p)$ s.t. $t_p.a = t_b.b$.
Such a join condition can also be used with the exploration join, as $R_b \; \vec{\bowtie}^{\; p_1}_{\; \psi_L(p_0).a \;  \ni \; b}  \; [R_p]$ shown in Figure~\ref{fig-operator}(b) where such a condition is evaluated in a nest-loop manner.
When each tuple $t_{p1} \in R_{p1}$ in Figure~\ref{fig-operator} has been enumerated, it would then iterate over all tuples in the other table, i.e. $R_{p0} = \psi_L (t_b.p_0)$, to find whether there is at least one tuple contains the same value.
If so, join $t_b$ and $t_p$ together.
\warn{Intuitively speaking, utilizing the explorational join condition with the exploration join together
would intersect the tuple sets pointed by pointers in different field, as $p_0$ and $p_1$ in Figure~\ref{fig-operator}(b).}

Similar to the standard ones in RDBMS, the introduced join condition can also have multiple physical implementations for a same logical one.
To execute the same join and evaluate the same exploration join condition in a hash manner as demonstrated in Figure~\ref{fig-operator}(c), a hash table would be first constructed for the table to be probed, i.e. $R_{p1}$ in Figure~\ref{fig-operator}, the constructed table can be reused when different pointers point to the same table.
As shown in Figure~\ref{fig-operator}, when each pointer is enumerated in field $p_0$, it would be first checked whether there has already been an existing hash table constructed for it.
If such a hash table has already been generated, it can be reused without reconstruct a new one.
Such a situation can happen in graph pattern matching in the pipeline intermediate relations when a same vertex appears multiply times in one same match or different matches.

Considering such a condition in the operator allows columns from different tables pointed by different pointers to be intersected without actually join them together.
It can be seen that an additional join would be required for the operation $R_b \; \vec{\bowtie}^{\; p_1}_{\; \psi_L(p_0).a \;  \ni \; b}  \; [R_p]$ demonstrated in Figure~\ref{fig-operator}(b) and (c) to be performed equivalently with the conventional relational operators.
Such an intersection is the basic component of the pattern matching algorithms~\cite{huang2014query, cordella2004sub, han2019efficient, han2013turboiso, bhattarai2019ceci, bouhenni2021survey, yang2021huge}, 
and such an introduced exploration join condition allows it to be evaluated seamlessly with the conventional relational algebra in a pipelined~\cite{boncz2005monetdb} manner, which would be demonstrated in Section~\ref{subsec-hybrid-query-execution}. 
Section~\ref{subsec-optimization} can further show that it is such an operation allows the \ModelName query to outperform the equivalent relational query.

\eat{(add it here?)}
It can also be easily seen that the various graph index construction methods~\cite{han2019efficient, bhattarai2019ceci, sun2020memory} can be directly plugged in here, by simply replace the base relations the operators directly gets from.

A \emph{resolution join} is also introduced as an operator in the query plan to consider the dynamic \emph{``relation-relation''}, \emph{``graph-relation''} and \emph{``graph-graph''} entity resolution to support \SQLd.
The \emph{``graph-relation''} entity resolution demonstrated in Figure~\ref{fig-operator} would first obtain all the matching result of pattern in the data graph, obtain all the attribute it needs and organized them as a relation.
\SystemName would then call any of the well-developed ER algorithms~\cite{binette2022almost} to resolve the entities across the two relations and join the tuple pairs that match with each other.

Principally speaking, the WCOJ (worst case optimal join)~\cite{ngo2018worst, mhedhbi2019optimizing, nguyen2015join, aberger2017emptyheaded, ngo2014skew} methods can also be considered here, 
in a similar way as previous works that integrate the WCOJ with the conventional join~\cite{wang2023free}.
Since we concentrate on the capability to process relation-graph hybrid query with \ModelName model here, there would not be an in-depth discussion of them here.

\eat{
Principally speaking, after representing both the \emph{relation} and \emph{graph} with the unified \ModelName model, 
there would be no need to distinguish which part of data is \emph{relational} and which part is \emph{graphic}.
However, after all, it is not how the users actually view the data and write the query.
This section would discuss how a query written in the SQL extension from Section~\ref{subsec-sql-extension} 
can be eventually rewritten to a query plan and then executed,
and how the unified plan space here can support a seamless evaluation for those hybrid query.

As the graph-relation query mapping itself has been well-studied in previous works~\cite{sun2015sqlgraph, blakeley2006ado, o2008object, bergmann2012applying, steer2017cytosm, vidal2017computing, xirogiannopoulos2017graphgen, boncz2018g, jindal2014graphiql},
while there are also works introduce operator for semantic connection to the relational query~\cite{TriQL, agrawal2009trio, altwaijry2015query, bhattacharya2006query, sismanis2009resolution},
the following discussion would directly face the query on the \emph{``relational view''} from Section~\ref{subsec-relational-view}.

It should be noticed that such a simplification here does not make the SQL extension in Section~\ref{subsec-sql-extension} worthless,
which is still meaning for users to properly query what they want.

This section would show how the \ModelName model can process the hybrid query written in the extended SQL demonstrated in Section~\ref{subsec-sql-extension}, with three stages:
(1) \emph{query mapping}, to map the hybrid query onto the \emph{relational interface} demonstrated in Figure~\ref{fig-overview}; 
(2) \emph{query rewrite}, to rewrite the query plan on the \emph{relational view} for it to execute on the \ModelName model; 
(3) \emph{optimization \& execution}, to generate an optimal plan and execute it.

Especially considering that the proposed \ModelName allows the graph and relational data to be described with both homogeneous data store and execution engine, 
it therefore allows an in-depth fusion of them as would be demonstrated in Section~\ref{subsec-optimization-and-execution} which can much benefit the \ModelName-based relation-graph polyglot system.

allows the graph and relational data to be represented within a same model, for the query across them to be considered with a unified plan space and executor for efficient improvement.

Meanwhile, since such a \emph{``relational view''} is deployed here as query interface, 
the upper level hybrid query would also be mapped to relational query first to convenient the query rewrite in Section~\ref{subsec-query-rewrite}.
As the graph-relation query mapping itself has already been studied in previous works~\cite{sun2015sqlgraph, blakeley2006ado, o2008object, bergmann2012applying, steer2017cytosm, vidal2017computing, xirogiannopoulos2017graphgen, boncz2018g, jindal2014graphiql},
it would be mainly focused on how the semantic connection in the hybrid query.


Different from the previous works that map the query on graph to relational algebra~\cite{sun2015sqlgraph, blakeley2006ado, o2008object, bergmann2012applying, steer2017cytosm, vidal2017computing, xirogiannopoulos2017graphgen, boncz2018g, jindal2014graphiql},
the operator to consider the semantic connection, \textcolor{red}{MAP} introduced in the SQL extension in Section~\ref{subsec-sql-extension}, is also required to be considered here. 
As~\cite{altwaijry2015query} has already demonstrated how such a kind of operator, polymorphic operators in their work, can be added in the join tree, therefore only the mapping process itself would be considered here.
}

\begin{figure*}[t]
	\vspace{-1.4ex}
	\centerline{\includegraphics[scale=1.3]{./fig/fig-hybrid-query-embedded.pdf}}
	\centering
	\vspace{-2.4ex}
	\caption{A demonstration of the hybrid query execution process with \ModelName model.}
	\label{fig-hybrid-query}
	\vspace{-3ex}
\end{figure*}

\subsection{Hybrid Query Plan}
\label{subsec-query-graph}

The mainstream query optimization workflows~\cite{moerkotte2008dynamic, bhargava1995hypergraph} for RDBMS basically all based on the query graph~\cite{abiteboul1995foundations}. 
The \ModelName model also provides a unified query graph to take all the introduced operators into consideration, for the entire existing optimization workflow to be inherited in \SystemName for hybrid query with minor modification as stated in Section~\ref{sec-overview}.
The hybrid query across the graph and relational data can then be optimized within a larger unified plan space to not miss the optimal one\textcolor{red}{(, as in Example.\ref{exa-running})}.

\eat{	It would be shown here in this section the query plan of the \ModelName model can also describe the access on both kinds of data in an unified space to support the evaluation of hybrid queries and the optimization of them.
	
	Introducing the above operators into the query plan allows the access on graph and relational data to be represented uniformally in the \ModelName query graph.
	The classic hypergraph-based query optimization workflow~\cite{moerkotte2008dynamic, bhargava1995hypergraph} can then be inherited in \SystemName with minor modification as demonstrated in Section~~\ref{subsec-overview}, for the hybrid query across graph and relational data with resolution join.
}

\eat{
	(To show: 
	(1) how the exploration join can be represented in the query graph; 
	(2) how the query graph allows the exploration to be considered from both sides;
	(3) how the query graph-based plan enumeration methods can be adopted.
	Describe them with an algorithm.)
}

The \ModelName query graph departs the conventional one for the standard relational query in two ways: 
directed edges for exploration join; and redundancy introduced on purpose to enlarge the plan space.
As mentioned previously in Section~\ref{subsec-RX-model-operator}, 
the introduced exploration join can only be explored through one direction, 
which thus required to be resolved to directed edges in the \ModelName query graph as demonstrated in Figure~\ref{fig-hybrid-query}, instead of being undirected for the conventional relational join.
In this case, the existing hypergraph-based query plan enumeration algorithms~\cite{moerkotte2008dynamic, bhargava1995hypergraph} can still be directly adopted here to enumerate all non-duplicated CSG (\underline{C}onnected \underline{S}ub\underline{G}raph)~\cite{moerkotte2008dynamic} pairs 
by simply treating all edges in the query graph are undirected.
If an enumerated pair of CSGs are connected by the exploration edges, an exploration join operator between them would then be generated according to the direction of those edges.

As a characteristic of the pointer introduced in \ModelName model, it should also be noticed that joining different tuples together and select a set of fields from them can break the pointers point to those tuples, especially when the joined result would be copied into another relation holding the intermediate result in the pipelined execution manner~\cite{boncz2005monetdb}.
For this reason, for each CSG pair enumerated for exploration join, all the exploration edges need to point to a CSG with only one vertex to ensure the pointer would not be invalided when the exploration join is being executed.
It can be seen that such a restriction naturally holds when the query plan is restricted to left-deep tree and there are always legal plans for pattern matching in the \SQLd query.
The enumerated CSG pairs would be first checked whether satisfy such a restriction to generate a legal exploration join.

Meanwhile, some redundancy would also be introduced when constructing the \ModelName query graph on purpose,
which then allows the exploration direction to be selected as in previous native graph-based pattern matching algorithms~\cite{huang2014query, cordella2004sub, han2019efficient, han2013turboiso, bhattarai2019ceci, bouhenni2021survey, yang2021huge}. 
Taking the \SQLd query in Figure~~\ref{fig-hybrid-query} as an intuitive example here,
it can be seen that the edge: $(v2)-[e1] \to (v1)$
can be explored equivalently in two opposite directions: from $v2$ through outward edge to $v1$; or from $v1$ through inward edge to $v2$.
Figure~\ref{fig-hybrid-query} shows that 
a redundancy would be introduced, as demonstrated by step (2), for these two directions to be both considered in the query graph\eat{, as path $(V_2)-[E_{1a}] \to (V_1)$ and $(V_1)-[E_{1b}] \to (V_2)$ respectively,} and only one of them would be preserved in each generated query plan.
The plan space would then be enlarged for an optimal exploration direction to be selected
with the cost model that would be given in Section~\ref{subsec-optimization}.

\eat{
	\revise{
		For the two CSGs connected by the edge of exploration join, they can be distinguished as one on the \emph{inward} side and the one on the \emph{outward} side.
		Since the exploration join edge can only be explored through one direction, the CSG on the outward side of the exploration edge would be constructed as the table to be explored defined in Section~\ref{subsec-RX-model-operator}.
		Meanwhile, each enumerated CSG pair would be checked whether is legal to be rewritten as a \ModelName query plan.
		Joining different tuples and move the joined data into the pipeline intermediate result can break the pointers point to them \textcolor{red}{(Needs more explanation?)}, therefore, the data can be.
	}
	
	Such a property would also be reflected in the \ModelName query graph.
	While the conventional relational query graph can be resolved to undirected edges, the exploration-join needs to be represented as directed edges in the query graph as demonstrated in Figure~\ref{fig-hybrid-query}.
	It can be easily seen that, by simply treating those directed edges in \ModelName query graph as undirected as they were in the conventional relational query graph, the existing hypergraph-based query plan enumeration algorithms~\cite{moerkotte2008dynamic, bhargava1995hypergraph} can be easily adopted here with minor modification.
	
\begin{myfloat}[t]
	%\vspace{-2.8ex}
	\hspace*{-1ex}
	\begin{minipage}{0.478\textwidth}
		\removelatexerror
		%\small
		%\setlength{\floatsep}{0cm} % set blank space above the figure
		%\setlength{\textfloatsep}{-10cm}% set blank space below the figure
		\IncMargin{0.2em}
		\LinesNotNumbered
		{\small
			\begin{algorithm}[H]
				\SetArgSty{textrm}
				\caption{\ModelName query graph construction process}
				\label{alg-sample}
				\Indentp{-2.5ex}
				\KwIn{\revise{An $\A$-graph $G_\A$},
					%\wrt an application $\A$,
					a positive integer $N$, two sampling strategies $M_v$ and $M_s$, and sample 
					ratios $\rho_v\%$ and $\rho\%$.}
				\KwOut{\revise{A set $H$ of} $N$ sample graphs $H_{(\A, \rho\%)}$.} %%
				\Indentp{1.4em}
				\nextnr
				$i \la 0$; \hspace{2ex} $H \la nil$\;
				\nextnr
				\Repeat{$i = N$}
				{
					\nextnr
					$\C \la nil$\;
					\nextnr
					\ForEach{predicate $p_0$ involved in $\A$}
					{
						\nextnr
						$\C \la \C \cup \PS(p_0, G_\A)$;}
					\nextnr
					$S_\A \la \PSample(\C, M_v, G_\A, \rho_v\%)$\;
					\nextnr
					$H_{(\A, \rho\%)} \la \LSample(S_\A, M_s, G_\A, \rho\%)$\;
					\nextnr
					$H \la H \cup \{H_{(\A, \rho\%)}\}$\;
					\nextnr 
					$i \la i + 1$\;
				}
				\nextnr
				\Return $H$;
				%\vspace{-0.2ex}
			\end{algorithm}
		}
	\end{minipage}
	\vspace{-2.7ex}
\end{myfloat}

\begin{myfloat}[t]
	%\vspace{-2.8ex}
	\hspace*{-1ex}
	\begin{minipage}{0.478\textwidth}
		\removelatexerror
		%\small
		%\setlength{\floatsep}{0cm} % set blank space above the figure
		%\setlength{\textfloatsep}{-10cm}% set blank space below the figure
		\IncMargin{0.2em}
		\LinesNotNumbered
		{\small
			\begin{algorithm}[H]
				\SetArgSty{textrm}
				\caption{\ModelName query graph construction}
				\label{alg-sample}
				\Indentp{-2.5ex}
				\KwIn{Logical \ModelName query plan.}
				\KwOut{\ModelName query graph.} %%
				\Indentp{1.4em}
				\nextnr
				\eat{
				$i \la 0$; \hspace{2ex} $H \la nil$\;
				\nextnr
				\Repeat{$i = N$}
				{
					\nextnr
					$\C \la nil$\;
					\nextnr
					\ForEach{predicate $p_0$ involved in $\A$}
					{
						\nextnr
						$\C \la \C \cup \PS(p_0, G_\A)$;}
					\nextnr
					$S_\A \la \PSample(\C, M_v, G_\A, \rho_v\%)$\;
					\nextnr
					$H_{(\A, \rho\%)} \la \LSample(S_\A, M_s, G_\A, \rho\%)$\;
					\nextnr
					$H \la H \cup \{H_{(\A, \rho\%)}\}$\;
					\nextnr 
					$i \la i + 1$\;
				}
				\nextnr}
				\Return $H$;
				%\vspace{-0.2ex}
			\end{algorithm}
		}
	\end{minipage}
	\vspace{-2.7ex}
\end{myfloat}


\begin{myfloat}[t]
	%\vspace{-2.8ex}
	\hspace*{-1ex}
	\begin{minipage}{0.478\textwidth}
		\removelatexerror
		%\small
		%\setlength{\floatsep}{0cm} % set blank space above the figure
		%\setlength{\textfloatsep}{-10cm}% set blank space below the figure
		\IncMargin{0.2em}
		\LinesNotNumbered
		{\small
			\begin{algorithm}[H]
				\SetArgSty{textrm}
				\caption{\ModelName query plan rewrite}
				\label{alg-sample}
				\Indentp{-2.5ex}
				\KwIn{\ModelName query graph.}
				\KwOut{Logical \ModelName query plan.} %%
				\Indentp{1.4em}
				\nextnr
				\eat{
				$i \la 0$; \hspace{2ex} $H \la nil$\;
				\nextnr
				\Repeat{$i = N$}
				{
					\nextnr
					$\C \la nil$\;
					\nextnr
					\ForEach{predicate $p_0$ involved in $\A$}
					{
						\nextnr
						$\C \la \C \cup \PS(p_0, G_\A)$;}
					\nextnr
					$S_\A \la \PSample(\C, M_v, G_\A, \rho_v\%)$\;
					\nextnr
					$H_{(\A, \rho\%)} \la \LSample(S_\A, M_s, G_\A, \rho\%)$\;
					\nextnr
					$H \la H \cup \{H_{(\A, \rho\%)}\}$\;
					\nextnr 
					$i \la i + 1$\;
				}
				\nextnr
				}
				\Return $H$;
				%\vspace{-0.2ex}
			\end{algorithm}
		}
	\end{minipage}
	\vspace{-2.7ex}
\end{myfloat}

\revise{
(To show: 
(1) Using the \emph{join order rule} to avoid generate multiply exploration join edge between two CSGs; 
(2) Restrict the CSG on the outward side to contain only one vertex in the query graph, to avoid the join of table break the pointers point to them;
(3) Introduced duplicated vertex in the query graph but would not contain duplicated vertices in the enumerated CSG pairs) \textcolor{red}{(Needs to be explained so detail?)}
}

\textcolor{red}{
Restrictions:
A pointer cannot point to a joined query vertex set;
}

\textcolor{red}{
Optimizations:
(1) Duplicate vertex needs no be generated;
(2) Several exploration join edge can be constructed as exploration join condition, instead of being constructed as another join;
}

\revise{
As mentioned previously in Section~\ref{subsec-RX-model-operator}, 
the introduced exploration join has more restrictions compared to the conventional relational ones.
Those restrictions can be easier seen in the query graph demonstrated in Figure~\ref{fig-hybrid-query}.
Considering a CSG pair: $\{\}$
}

\revise{
A set of join order rules can be used to generate a legal query tree through plan enumeration.
The previous section 
As shown in Figure~\ref{fig-hybrid-query}, once an edge table is explored in the query graph, the outward exploration edge toward the dst/src field would then be explored to add the connected vertex table into the query tree.
Meanwhile, several vertices in the query graph can be considered equivalently as the exploration join condition instead of being another join operator, e.g. the $E_{2b}$ in Figure~\ref{fig-hybrid-query}.
As can be seen in the query tree  in Figure~\ref{fig-hybrid-query}, only one query graph vertex would be explored in each join step, and there would be only one exploration edge connects two CSGs.
Such a rule can make the 
}

\revise{
For the two CSGs connected by the edge of exploration join, they can be distinguished as one on the \emph{inward} side and the one on the \emph{outward} side.
Since the exploration join edge can only be explored through one direction, the CSG on the outward side of the exploration edge would be constructed as the table to be explored defined in Section~\ref{subsec-RX-model-operator}.
Meanwhile, each enumerated CSG pair would be checked whether is legal to be rewritten as a \ModelName query plan.
Joining different tuples and move the joined data into the pipeline intermediate result can break the pointers point to them \textcolor{red}{(Needs more explanation?)}, therefore, the data can be.
}
}

\eat{
	Except some edges are directed, another main difference between the \ModelName query graph and the conventional one is there can be vertices duplicate to each other and only one of them needs to be considered in the generated query plan.
	Such a \emph{duplicate \& deduplicate} process allows a larger plan space to be considered without generating redundant constraints in the query plan.   
	Taking the $SQL_D$ query in Figure~~\ref{fig-hybrid-query} as an intuitive example here,
	it can seen the path: $[v2]-[e1]->(v1)$
	can be explored equivalently in two opposite directions: from $v2$ through outward edge to $v1$; or from $v1$ through inward edge to $v2$,
	and only the one with lower cost between them needs to be preserved in the generated plan.
	
Corresponding to the three steps demonstrated in Figure~~\ref{fig-hybrid-query}, 
the \ModelName query graph construction and plan enumeration process can be described as follow:
(1) Construct query graph.
(2) Construct duplicate edge.
(3) Enumerate CSG (\underline{C}onnected \underline{S}ub\underline{G}raph)~\cite{moerkotte2008dynamic} pairs without duplicated vertex.
Where CSG pairs enumeration process can adopt any of the existing algorithms.

To formally describe such a kind of duplication, we introduce duplicate rule as:

\textcolor{red}{
	\etitle{Duplicate rule}. Duplicate rules set $\Sigma$.
}

\begin{example}
	\label{example-schema-info}
	The equivalence between the two queries, (\ref{logical_query_x_y_z}) and (\ref{logical_query_z_y_x}) in Example.\ref{example-plain_matching} can be described with the schema information $\Sigma$:
	\begin{align*}
		\forall x \in V, \forall y \in \psi_L(\psi_L(x._{out})._{dst})
		&\to x \in \psi_L(\psi_L(y._{in})._{src}) \\
		\forall x \in V, \forall y \in \psi_L(\psi_L(x._{in})._{src}) 
		&\to x \in \psi_L(\psi_L(y._{out})._{dst})
	\end{align*} 
	which suggest that for any vertex $x$ and $y$, if there exists an output edge of $x$ toward $y$, then there exists an input edge of $y$ from $x$, vice versa. The equivalence between (\ref{logical_query_x_y_z}) and (\ref{logical_query_z_y_x}) can easily be seen.
\end{example}

}

\eat{(To explain that $E_{2b}$ is not constructed as a vertex in graph?)}

It can be seen from the generated physical query plan demonstrated in Figure~\ref{fig-hybrid-query} that joining with conventional relations can take place in any order: in ahead, in the middle or after matching the graph pattern,
which can be supported by the seamless execution process that would be shown in Section~~\ref{subsec-hybrid-query-execution}.
Such an enlarged plan space can then take the optimal query plan into consideration, which would be shown with the cost model in Section~\ref{subsec-optimization}.

Since the \emph{resolution join} operator itself can only be regarded as a black-box here, there cannot be any guarantee for it to be moved through the query tree without influence the eventually query result.
It would then be handled in a similar but more restricted way as the \emph{``aggression''}~\cite{galindo2001orthogonal} in the conventional relational query plan.
Optimized query tree would be generated for each child of the \emph{resolution join operator} separately. 
The output of the \emph{resolution join operator} would then be regarded as a base relation in the query graph for further optimizations.

More optimization methods can be considered for the \emph{resolution join operator} if more properties of the resolution process can be guaranteed \textcolor{red}{(would be considered in following work)}.


\eat{
\begin{figure}[t]
\vspace{-1.4ex}
\centerline{\includegraphics[scale=1.6]{./fig/fig-execution.eps}}
\centering
\vspace{-2.4ex}
\caption{A demonstration of the query execution process of physical plan 0. }
\label{fig-execution}
\vspace{-3ex}
\end{figure}
}


\subsection{Hybrid Query Execution}
\label{subsec-hybrid-query-execution}

It is shown previously that introducing the operators to the \ModelName query plan allows the access on relational and graph data to be represented in a unified plan space.
Since the cross model access has been eliminated in the very beginning by utilizing the \ModelName model, 
it would be shown here that the hybrid query plan can then be executed seamlessly, accessing across both kind of data without blocking the pipelined execution~\cite{boncz2005monetdb} process.

\eat{
(To show: 
	(1) the exploration join can be executed in a pipelined manner; 
	(2) it can be integrated into the pipeline execution process without cost.)
}

We first show that the introduced exploration join can also be executed in a pipelined manner~\cite{boncz2005monetdb}, instead of the typical exploration process in the pattern matching algorithms~\cite{huang2014query, cordella2004sub, han2019efficient, han2013turboiso, bhattarai2019ceci, bouhenni2021survey, yang2021huge} which basically corresponds to the volcano model~\cite{graefe1993volcano} in the field of RDBMS.
As demonstrated in the pipeline execution process of the exploration join in the rightest part of Figure~\ref{fig-hybrid-query}, 
it would first iterate all tuples in the pipeline intermediate result and explore from the pointer in field $V_0.out$, iterate over all tuples it points and copy the $dst$ field of it into the pipeline intermediate result in next stage.
It can be seen that coping a pointer from one table to another here would not invalid it,
which can thus allow the pipeline keep running for next operator.
It can also be seen that other existing execution optimizations in RDBMS~\cite{menon2017relaxed,neumann2011efficiently} can also be utilized to further improve its performance,
\warn{which are rarely considered in the native graph-based pattern matching algorithms}.

\eat{
	An example of a typical pipeline execution process is demonstrated in the rightest side of Figure~\ref{fig-hybrid-query}.
	As an extension of the classic relational model, the conventional relational operators would be executed equivalently as they were in previous typical relational engine.
}

Meanwhile, it can be seen that such an execution process can integrate the exploration join and conventional join together in the pipeline executor uniformly.
The pointers to be explored, $v_0.out$ and $v_1.in$, would be first copied into the pipeline intermediate result from the field $out_L$ in vertex table.
After that, in $step_2$, the pointers in the intermediate result can then be used for exploration and intersection, e.g. find whether a candidate for the pattern graph to match is also the inward/outward edge of several vertices that have already been matched onto the data graph, runs in the graph pattern matching algorithm. 

The introduced \emph{resolution join} would become a pipeline breaker in the execution process.
Since the \emph{resolution process} can only be regarded as a black box, instead of waiting only for the pipeline intermediate to be filled, 
the execution of the \emph{resolution join} also cannot be reordered, which needs to wait until all results of its both child have been obtained.
Optimization methods can be considered to execute the \emph{resolution join} approximately to avoid generate enormous intermediate results \textcolor{red}{(which would be considered in following work).}


\eat{
\textcolor{red}{Figure~\ref{fig-hybrid-query} shows how the exploration on graph data can be integrated into the executer from~\cite{boncz2005monetdb}}

Figure~\ref{fig-hybrid-query} shows how the exploration on graph data can be integrated into the executer from~\cite{boncz2005monetdb}

\textcolor{red}{The semantic join would be considered as a non-reorderable operator in the pipeline.}

\textcolor{red}{The exploration join demonstrated in Figure~\ref{fig-hybrid-query} cannot be considered in the conventional relational join plan and it can be seen
	in the following subsection of estimation that such an operation can bring efficiency improvement.
}}

\subsection{Hybrid Query Plan Cost Estimation}
\label{subsec-optimization}

To support a cost-based optimization for the hybrid query, the cost estimation strategises for the conventional relational query is also inherited and extended here to take the introduced operators into consideration.
It can also be shown with the estimated cost that the enlarged plan space in \ModelName model allows the optimal query plan to be considered for hybrid query, comparing to access graph and relational data separately.

\eat{
(To show: 
(1) the previous relational cardinality estimation methods can be directly utilized here; 
(2) the cost of exploration join operator can be estimated by the extended cost model; 
(3) use the cost model to show that the enlarged unified plan space allows more efficient plan to be considered.)
}

The cost of an enumerated plan can be estimated with cardinality estimation and a cost model to evaluate each operator.
It has been stated in Section~\ref{sec-overview} that the cardinality for querying the data with \ModelName model can be estimated with existing methods,
whether the conventional ones for RDBMS~\cite{cormode2011synopses, harmouch2017cardinality, leis2017cardinality, park2020g, kim2021combining,yang2021huge, perron2019learned} or the ones specifically developed for graph pattern matching ~\cite{park2020g, kim2021combining}.
As an intuitive explanation of how they can be directly adopted here, it can be seen that matching the same pattern on the same data graph would generate a same number of matching, whether through the relation-based methods or the native graph-based methods.

As also demonstrated in Figure~\ref{fig-overview}, only the cost model requires to be extended to take the newly introduced operators into consideration.
Since all the operators in conventional relational query plan would be preserved in the \ModelName model, 
it would be only necessary for the existing cost model~\cite{leis2015good, manegold2002generic} to be extended to consider the newly introduced operators, instead of developing one from sketch.
To show how the cost to execute the introduced operators can be estimated, $C_{mm}$ proposed in~\cite{leis2015good} is extended as $C_{lmm}$ here, as:
\begin{equation*}
	C_{lmm}(Plan) = \Sigma_{op \in Plan}  E_{times}(op) * E_{cost}(op) 
\end{equation*}
As the execution process of the physical operator demonstrated in Section~\ref{subsec-RX-model-operator}, the introduced operate also consists of the basic components of nest-loop iteration and hash table.
\begin{align*}
	C_{lmm}(T) = 
	\begin{cases}
		C_{mm}(T)              & \text{(if $T = T_1 \bowtie_{inl} T_2$)}  \\
							   & \text{(or $T = T_1 \bowtie_{hj} T_2$ or $T = R$)} \\
		\tau |T_1| \times |\psi_L(T_1.p)|   & \text{(if $T = T_1 \vec{\bowtie}^{ \; p} \; [T_2]$)}  \\
		\intertext{$\tau |T_1| \times |\psi_L(T_1.p_1)| \times ( 1 + |\psi_L(T_1.p_0)|)$}
		& \text{(if $T = T_1 \vec{\bowtie}^{ \; p_1}_{\; inl(\psi_L(p_0).a \;  \ni \; b)} \; [T_2]$)}  \\
		\intertext{$\tau |T_1| \times (|\psi_L(T_1.p_1)| + |\psi_L(T_1.p_0)|) + |T|$}
		& \text{(if $T = T_1 \vec{\bowtie}^{ \; p_1}_{\; hj(\psi_L(p_0).a \;  \ni \; b)} \; [T_2]$)} 
	\end{cases}    
\end{align*}
Same as in~\cite{leis2015good}, $\tau \leq 1$ represents the cost of table scan compared to the lookup in hash table,
while $\lambda$ denotes the relative cost of lookup in index.

\begin{example}
	\label{example-cost-model}
	For the \SQLd in Figure~\ref{fig-hybrid-query}, we provide three typical query plans and evaluate their cost with the proposed cost model $C_{lmm}$. For a simplification, the edge relations would be all omitted in the following description.
	
	The three query plan here join the relation $R$ in different order and all use the \emph{hash join} and \emph{hash explorational join condition}: $P_{RF}$, to first join the relational data and explore the vertex: $\{R, V_0, V_1, V_2\}$ in order;
	$P_{GF}$, to first match the graph pattern and explore the vertex: $\{V_0, V_1, V_2, R\}$ in order;
	$P_{H}$, to first obtain a partial match of the pattern, then join it with the relation, and finally complete the entire match of the pattern, which would explore : $\{V_0, V_1, R, V_2\}$ in order.
	With the introduced $C_{lmm}$, there would be:
	\begin{align*}
		C_{lmm}(P_H)  &= \tau |V_0| + \tau |V_0 V_1| + |V_0 V_1 R| + \tau |R| + \tau |V_0 V_1 V_2 R| \\
		C_{lmm}(P_{RF}) &= \tau |V_0| + \tau |R| + |V_0 R| + \tau |V_0 V_1 R| + \tau |V_0 V_1 V_2 R| \\
		C_{lmm}(P_{GF}) &= \tau |V_0| + \tau |V_0 V_1| + \tau |V_0 V_1 V_2| + \tau |R| + |V_0 V_1 V_2 R|
	\end{align*}
	Where $| ... |$ denotes the cardinality of a subquery, represented by a subset of the vertices in the query graph.
	
	In align with the setting in~\cite{leis2015good}, we also set $\tau = 0.2$ and $\lambda = 2$ here. 
	Assume that in a given data graph there are $|V_0 V_1| < |V_0| < |V_0 V_1 V_2|$, intuitively, it means for each vertex matched for $V_0$ in the data graph, 
	it is not likely to find a vertex connect to it to match for $V_1$;
	However, once both $V_0$ and $V_1$ are matched on the data graph, there can be lots of vertex to match for $V_2$.
	
	To actually calculate a cost of the above three plans, we can setting the cardinality of those subqueries as follow:
	$|V_0|         = 1000$,
	$|V_0 V_1|     = 100$,
	$|V_0 V_1 V_2| = 2000$,
	$|R|             = 1000$,
	$|V_0 R|         = 10000$,
	$|V_0 V_1 R|     = 1000$,
	$|V_0 V_1 V_2 R| = 20000$. One can easily verify that such a data graph can be constructed.
	\eat{
		C_{lmm}(P_H)    &= 200 + 20  + 1000  + 200 + 4000  = 5420  \\
		C_{lmm}(P_{RF}) &= 200 + 200 + 10000 + 200 + 4000  = 14600 \\
		C_{lmm}(P_{GF}) &= 200 + 20  + 400   + 200 + 20000 = 20820
	}
	We then have: $C_{lmm}(P_H) = 5420$, $C_{lmm}(P_{RF}) = 14600$ and $C_{lmm}(P_{GF}) = 20820$. It can be seen that $C_{lmm}(P_H) \approx 0.37 \; C_{lmm}(P_{RF}) \approx 0.26 \; C_{lmm}(P_{GF})$, which means neither to join all relation in ahead nor match the graph pattern in ahead can be the most optimal query plan.
\end{example}

Materialization strategies~\cite{perron2019learned} \textcolor{red}{(not implemented yet)} would be utilized for estimating the cardinality of entity resolution. 


\eat{
\begin{figure}[t]
	\vspace{-1.4ex}
	\centerline{\includegraphics[scale=1.6]{./fig/fig-physical-query.eps}}
	\centering
	\vspace{-2.4ex}
	\caption{(a) to (d): Different physical query plans for  $Q_2$ in Figure~\ref{fig-pattern-graph-example}(a). 
		(e) to (g) Pseudo-code for the physical plan from (a) to (c). }
	\label{fig-physical-query}
	\vspace{-3ex}
\end{figure}}

\vspace{-0.4ex}


==> sec-maintenance.tex <==
\vspace{-0.3ex}
%%%%%%%% Section 1 %%%%%%%%

\section{maintenance}
\label{sec-maintenance}

\warn{
	It has been long attacked~\cite{stonebraker2005goes} that the \emph{``link''} in the \emph{``network model''}~\cite{DBTG1971CODASYL} is unmaintainable 
	which also breaks the physical data independence~\cite{stonebraker1975implementation}.
	Different from previous works~\cite{DBTG1971CODASYL},
	the modification on the \ModelName model is still defined on the logic-level in a similar way as the pointers
	introducedin Section~\ref*{subsec-define-model}.
	
	In this section, it would be shown how a modification, 
	conceptionally in the graph structure,
	can be converted to a series of pointer reattachment and tuple modification that can be directly supported by the 
	mechanisms shown in Section~\ref{subsec-physical-implementation}.
}


% Although the \ModelName model provides an equivalent representation for the graph data, it still needs to be browsed in the graph structure for an intuitive recognition to write the \SQLd query.
% \eat{Meanwhile, the discussion about optimization and execution in Section~\ref{sec-hybrid-query-evaluation} also assumes that a query plan has already be given, which is still a gap from the input declarative \SQLd query.}
% \revise{Meanwhile, in an opposite direction, the updates of data that conceptionally in the graph structure
% 	also need to be rewritten onto the inner \ModelName-structured and to eventually modify the pointers as defined logically in Section~\ref{subsec-define-model}.} 
% A \revise{bidirectional} connection between the graph and the \ModelName model is thus in demand to support both these two requirements.

% In opposite of constructing graph view for relational data~\cite{xirogiannopoulos2017graphgen, da2020kaskade}, a \emph{virtual relational view} would be constructed as an intermediate representation that bridges the graph and \ModelName model for both graph browsing and \SQLd query parsing.
% \revise{Such a view would be only used for query rewriting and browsing and fundamentally has no need for materializing, 
% 	which avoids the massive detailed discussion of the view selection~\cite{chirkova2002formal, gupta1999selection} and materialization~\cite{goldstein2001optimizing,halevy2001answering,blakeley1986efficiently,dayal1978updatability,chirkova2012materialized}.
% }

% \subsection{View Conversion Rule}
% \label{subsec-from-relation-to-XXX-model}

\eat{
In Section~~\ref{subsec-from-relation-to-XXX-model}, we briefly shown how the Vertex and Edge table can be converted to the \ModelName data.

	\revise{
		\etitle{Definition}. Relational view of graph-structured data, e.g. vertex table and graph table.
	}
	
	\textcolor{red}{Here, we show how a graph represented by relations can be converted to the \ModelName model.}
	
	
	
	We assume that the graph data has been stored in a Vertex table and an edge table as shown in Figure~\ref{fig-relation}
	
	To formally describe the data conversion process, we define several conversion operator here:
}

% A set of view conversion rules would be first defined here to describe how the relational view can be constructed, which can be used in two directions for graph browsing and query parsing respectively as demonstrated in Figure~\ref{fig-view}.

% \etitle{View conversion rules}.
% {\small
% 	\begin{align*}
% 		\text{\d{$\vec{\ltimes}$}}:& \; \text{construct join index in lhs relation and partition rhs relation,} \\
% 		& \; \text{does not preserve the column to join in the rhs relation;}  \\
% 		\text{\d{$\vec{\rtimes}$}}:& \; \text{construct join index in lhs relation and partition rhs relation,} \\
% 		& \; \text{does not preserve the column to join in the lhs relation;}
% 	\end{align*}
% }

% The following example shows how a relational view can be constructed from the inner \ModelName data with the above rules:

% \begin{example}
% 	\textcolor{red}{(Need rewrite)} Given the conversion rule below:
% 	\begin{align*}
% 		\{Vertex_0, Vertex_1\} \, & \text{\d{$\vec{\ltimes}$}}_{vId = sId} \, \{Edge_0, Edge_1\}, \\ 
% 		\{Vertex_0, Vertex_1\} \, & \text{\d{$\vec{\ltimes}$}}_{vId = tId} \, \{Edge_0, Edge_1\}, \\
% 		\{Vertex_0, Vertex_1\} \, & \text{\d{$\vec{\ltimes}$}}_{vId = sId} \, \{Edge_0, Edge_1\} \, \text{$\vec{\rtimes}$}_{tId = vId} \, \{Vertex_0, Vertex_1\}, \\
% 		\{Vertex_0, Vertex_1\} \, & \text{\d{$\vec{\ltimes}$}}_{vId = tId} \, \{Edge_0, Edge_1\} \, \text{$\vec{\rtimes}$}_{sId = vId} \, \{Vertex_0, Vertex_1\} 
% 	\end{align*}
% 	We can construct the relational view in \tbf from the \ModelName-structured data in  \tbf.
% \end{example}

% The above rules can also be used reversely, from the relational view to inner \ModelName-structured data,
% to convert the data from graph to \ModelName structure, as in the following example:

% \begin{example}
% 	given a data graph, show how it can be converted to \ModelName structure:
% \end{example}


% Based on the relational view, the works of graph visualization~\cite{beck2017taxonomy, herman2000graph, antoniazzi2018rdf}, especially for RDF~\cite{RDF} data, can be directly utilized to browse the graph data stored in \ModelName model.
% Meanwhile, such a usage of the conversion rule also allows the query and modification on graph or relational view to be rewritten onto the \ModelName-structured data.

\eat{
	\begin{figure}[t]
		\centerline{\includegraphics[scale=0.8]{./fig/fig-hierarchy.eps}}
		\centering
		\vspace{-2.4ex}
		\caption{
			A demonstration of the hierarchy of different data models.}
		\label{fig-data-model}
		\vspace{-3ex}
	\end{figure}
}

% \begin{figure}[t]
% \vspace{-1.4ex}
% \centerline{\includegraphics[scale=2.0]{./fig/fig-view.eps}}
% \centering
% \vspace{-2.4ex}
% \caption{A demonstration of the relational view for query rewrite and data graph browsing.}
% \label{fig-view}
% \vspace{-3ex}
% \end{figure}

% \subsection{Modification Rewrite}
% \label{subsec-query-rewrite}

\eat{
It has been long attacked~\cite{stonebraker2005goes} that the \emph{``links''} in the network model~\cite{DBTG1971CODASYL} is unmaintainable 
which also breaks the physical data independence~\cite{stonebraker1975implementation}.
Different from previous works~\cite{DBTG1971CODASYL}, 
the explicit modification of the \emph{pointers} introduced in the \ModelName model is also defined on logic level, as:

\etitle{Pointer reattachment}. 
Considering a set of \emph{extended relations} $\D_L = (D_1, \ldots, D_n, \psi)$,
given a pointer $p \in \mathbb{P}$ and a tuple set $T \subseteq D_i$ $(1 \leq i \leq n)$,
the \emph{modification} of $p$ that re-attach it to $T$ is defined as: $\mathcal{M}(p, T, \psi) = \psi'$,
s.t. $\psi'(p) = T$, and $\psi'(p') = \psi(p')$ for $\forall p' \in \mathbb{P} \setminus \{p\}$.

Intuitively, the pointers here are allowed to be reattached to another set of tuples explicitly.
Meanwhile, principally speaking, introducing/removing a tuple to/from \ModelName-structured data
also suppose to modify all \emph{pointers} point to it in an implicited way.
However, generally speaking, it can be seen that the resources required to track all the pointers
that would be influenced for each tuple is unaffordable.

As a logic-level definition, the modification of the tuples in \ModelName model would bring undefined influence to 
all the pointers without providing automatic maintenance.
The correctness of the pointers would be guaranteed by the query rewrite procedural
that would be shown in Section~\ref{sec-maintenance}, 
from the one conceptionally in the graph structure to a series of explicit modifications of all related pointers, 
where the cost can be bounded by the locality of graph~\cite{yuan2012modeling, cong2006study}.

\eat{
The locality of the graph structure~\cite{yuan2012modeling, cong2006study}
allows the range of modification to be bounded.

Meanwhile, removing tuple from the relations would also bring modification to the pointers 
automatically, as:

\etitle{Tuple removel}. 
Given an \emph{extended relation} set $\D_L = (D_1, \ldots, D_n, \psi)$ 
and a tuple $t \in D_i$ $(1 \leq i \leq n)$,
removing $t$ from $D_i$ would also modify the \emph{pointers}, 
as: $\mathcal{M}_D(t, \psi) = \psi'$ 
s.t. $\psi'(p) = \psi(p) \setminus \{t\}$ for $\forall p \in \mathbb{P}$.

Intuitively, the pointers are allowed to be reattached to another set of tuples explicitly,
while removing a tuple from the relations would also automatically disconnect it 
with the \emph{pointers} point to it.
Section~\ref{subsec-physical-implementation} would show how various kinds of physical designs 
allows such a pointer and the modification of it to be implemented efficiently.
And Section~\ref{sec-maintenance} would show that how the updates, conceptionally in the graph structure, can be transformed onto the 
modification of the pointer, bridged by a \emph{virtual relational view}.}

}


\eat{
	Although the definition are unified for the all kinds of pointers, 
	they can still correspond to different physical implementations
	under different scenarios: to a single tuple; a subset of tuples in a table; a whole table, for the consideration of efficiency.
}

\eat{(Show how the modification can be done for different kinds of physical implementations.)}


\eat{
Introducing new vertex/edge to the graph data is relatively trivial.
As a comparison, the key challenge for graph structured data maintenance is to make sure 
all pointers are still valid after a tuple has been removed, which is defined as:

\etitle{Well-behaved tuple removel}. 
Given an \emph{extended relation} set $\D_L = (D_1, \ldots, D_n, \psi)$ 
and a tuple $t \in D_i$ $(1 \leq i \leq n)$,
removing $t$ from $D_i$ would also modify the \emph{pointers}, 
as: $\mathcal{M}_D(t, \psi) = \psi'$ 
s.t. $\psi'(p) = \psi(p) \setminus \{t\}$ for $\forall p \in \mathbb{P}$.

It can be checked that the following update rewrite procedural can garantee that the modification process to 
be well-behaved.
}

\warn{
(Describe how the modification can be rewritten onto the inner \ModelName-structured data).

\etitle{Insert Vertex \& Edge}.
Given a graph $G = (V_G, E_G, F_A)$ that has already been stored in \ModelName tables: 
$Vertex(vId, label, in_L, out_L)$,
$Vertex_{A}(vId, key_0, key_1, \dots)$,
$[Edge_{out}](eId, label, dst_L)$,
and $[Edge_{in}](eId, label, src_L)$.
Considering an incremetal on it 
$\Delta G_+ = (\Delta V_{G+}, \Delta E_{G+}, \Delta F_{A+})$,
which introduce a set of new vertices $\Delta V_{G+}$ and a set of new edges $\Delta E_{G+}$.
Similar to the graph data conversion process shown in Section~\ref*{subsec-define-model},
the introduced vertices and edges can be eventually converted onto \ModelName-structured data
in following steps:

(1) Introduce new tuples to relation $Vertex$ for each new vertices,
and tuples to relation $Vertex_A$ for the attribute of the new vertices,
set all fields up in a same way as the graph conversion in Section~\ref*{subsec-define-model}.

(2) Collect the new edges in $\Delta E_{G+}$ by their \emph{src} and \emph{dst},
\ie for $\forall v \in V_G \cup \Delta V_{G+}$, get a set of new edges outward from it:
$\Delta Edge_{out\_v} = \{e.src = v | e \in \Delta E_{G+}\}$ and a set of new edges toward it:
$\Delta Edge_{in\_v}  = \{e.dst = v | e \in \Delta E_{G+}\}$.

(3) Maintaince the table of in/out edges.
For each vertex $\forall v \in V_G \cup \Delta V_{G+}$, 
set the edge set $Edge_{out\_v}' = Edge_{out\_v} \cup \Delta Edge_{out\_v}$
and $Edge_{in\_v}' = Edge_{in\_v} \cup \Delta Edge_{in\_v}$.

(4) Connnect the in/out field of vertices in table $Vertex$ 
to the corresponding in/out edge table
if they were once $nullptr$,
\ie the newly introduced vertices or the vertices once does not have inward/outward edges at all.

During the above process, some table might needs to be resized and moved to another position, 
as described in Section~\ref*{subsec-physical-implementation}, 
utilizing the \emph{``indirected''} pointer allows the pointers still point to the corresponding table/tuple
after modification.
\textbf{A \emph{``directed''} pointer can be generated after all modification have been updated for a more efficient processing.}

\etitle{Remove Vertex \& Edge}. 
Similar to the insert process above.
}

% Through a well-studied query mapping process~\cite{sun2015sqlgraph, blakeley2006ado, o2008object, bergmann2012applying, steer2017cytosm, vidal2017computing, xirogiannopoulos2017graphgen, boncz2018g}, query in the extended SQL here can be mapped onto a relational interface,
% as can be seen from the query processing workflow that would be briefly demonstrated in Section~\ref{subsec-overview}.

% Similar to the previous works that rewrite the query on view~\cite{goldstein2001optimizing, halevy2001answering}.

% As the graph patten matching can be described with relational algebra equivalently~\cite{jachiet2020optimization, bancilhon1989amateurs, agrawal1988alpha, abiteboul1995foundations, melton2001sql, nguyen2015join, sun2015sqlgraph, blakeley2006ado, o2008object, bergmann2012applying, steer2017cytosm, vidal2017computing, xirogiannopoulos2017graphgen, boncz2018g, jindal2014graphiql},
% utilizing such a relational view as an intermediate query interface then allow us to make a use of the existing works of graph-relation query mapping~\cite{sun2015sqlgraph, blakeley2006ado, o2008object, bergmann2012applying, steer2017cytosm, vidal2017computing, xirogiannopoulos2017graphgen, boncz2018g, jindal2014graphiql} to avoid developing a parser from scratch.

% (Demonstrate arbitrary relational update on the relational view can be transformed on to the \ModelName model with the view construction rule.)

% With the conversion rules, query and modification on the relational view can be rewritten to the inner \ModelName structured data as shown in the example below:

% \begin{example}
% 	\label{exp-query-can-convert}
% 	Considering Figure~\ref{fig-relation}(a) as the relational view and Figure~\ref{fig-view}(a) as the actual data organization of it,
% 	the query plan (\ref{order_f_h_plan}) in Example.\ref{example-query-plan-order} can be converted to execute on the actual data organization as:
% 	\begin{align*}
% 		\forall a \in f, \forall b \in \psi_L(a.h_L) \to query(a.x, b.y)
% 	\end{align*}
% 	where the conversion rule $f \, \vec{\bowtie}_{x = x} \, h$ allows the exploration through the pointer $h_L$ to replace the value-based join represented by $a.x = b.x$. 
% 	The same logical query plan would also be generated similarly on the data organizations from Figure~\ref{fig-view}(b) to (d).
% \end{example}

% \revise{We can then define the query rewrite process as follow:}

% \etitle{Logical query plan rewrite}. 
% For a query plan:
% \begin{align*}
% 	\forall x \in f \; ... \; \forall y \in g \; ... \; x.a = y.b \; ...  
% \end{align*}
% If the \emph{conversion rule} of the view contains any of 
% $f \; \text{$\vec{\bowtie}$}_{a = b} \; g$,
% $f \; \text{$\vec{\ltimes}$}_{a = b} \; g$,
% $f \; \text{\d{$\vec{\bowtie}$}}_{a = b} \; g$ or
% $f \; \text{\d{$\vec{\ltimes}$}}_{a = b} \; g$, then it can be written as:
% \begin{align*}
% 	\forall x \in f \; ... \; \forall y \in \psi_L(x._{g_{a \to b}}) \; ... 
% \end{align*}
% if for $\forall c$, there is
% $g \; \text{$\vec{\ltimes}$}_{c = a} \; f$ or
% $g \; \text{\d{$\vec{\ltimes}$}}_{c = a} \; f$ contained in the \emph{conversion rule};
% or for $\forall c \neq a$, there is
% $f \; \text{$\vec{\ltimes}$}_{c = b} \; g$ or
% $f \; \text{\d{$\vec{\ltimes}$}}_{c = b} \; g$, then it cannot be converted to the query plan on the \ModelName-structured data.
% \\
% In other cases, the query plan remains the same.

% Such a replacement rule should be taken from right to left, as in a more complicated query:
% \begin{align*}
% 	\forall x \in f \; ... \; \forall y \in g \; ... \; x.a = y.b \; ... \; \forall z \in h \; ... \; y.c = z.d \; ...  
% \end{align*}
% where the conversion rule contains: 
% $f \; \text{$\vec{\ltimes}$}_{a = b} \; g$ and 
% $g \; \text{$\vec{\ltimes}$}_{c = d} \; h$, then it can be rewritten first as:
% \begin{align*}
% 	\forall x \in f \; ... \; \forall y \in g \; ... \; x.a = y.b \; ... \; \forall z \in \psi_L(y._{h_{c \to d}}) \; ...  
% \end{align*}
% then:
% \begin{align*}
% 	\forall x \in f \; ... \; \forall y \in \psi_L(x._{g_{a \to b}}) \; ... \; \forall z \in \psi_L(y._{h_{c \to d}}) \; ...  
% \end{align*}

% \textcolor{red}{...}

% \textcolor{red}{Here, we show how the update on the relational view can be transformed onto the inner data structure through the conversion rule.}

% Querying on the \emph{relation view} with the SQL, the composability of the query language can be naturally obtained which is inline with what~\cite{angles2018GCORE} advocates.


% % The discussion here would only briefly about how such a view is possible, the detailed query conversion and view construction methods would be given in Section~\ref{sec-logical-query-on-tbf-model} and  Section~\ref{sec-conversion} respectively.

% It would be discussed here how the update on view~\cite{dayal1978updatability, blakeley1986efficiently} can be 
% propagated to the inner data structure, as in~\cite{zaniolo1979design}, which is more convenient here.

% Assume there is an update on the relational view, we then demonstrate how it can be transformed onto the fragmented dataset through the \textcolor{red}{view construction rules}. 

% \begin{example}
% 	As the update demonstrated in Figure~\ref{fig-view}, 
% 	the inserted tuple on the view would be translated onto the internal data structure, where the related pointers would also be modified.
% 	The view construction rules here works in a similar way as the triggered rule system in \cite{stonebraker1990implementation, stonebraker1992integration, widom1996starburst,abiteboul1995foundations}.
% \end{example}

\vspace{-0.4ex}


==> sec-preliminary.tex <==
\vspace{-0.3ex}
%%%%%%%% Section 1 %%%%%%%%

\section{Preliminary}

\etitle{Relation model}.
Database can be regarded an interpretation of multi-ary predicates, as $f(x,y)$, $h(x,w,y)$ in Fig.\ref{fig-relation}(a).

\etitle{Relation algebra}.

\etitle{Graph}. 

\etitle{Graph data model}.

\etitle{Graph pattern matching}. 

\etitle{Relational graph data processing}. 

\eat{
Excepts the query language directly based on the native graph model~\cite{francis2018cypher, angles2017foundations, TinkerPop, openCypher}, 
lots of previous works also utilize SQL or its extensions with additional recursive features to describe the computational tasks on graph~\cite{ma2016g,zhao2019sql,zhao2017all,sparql}.
Especially from the relational perspective, pattern matching, one of the most widely considered tasks on graph~\cite{SahuMSLO2020ubiquity, hegeman2018survey, angles2018GCORE},
can actually be described with the standard relational algebra without any extension~\cite{nguyen2015join},
which therefore leads to previous works of relational graph data processing~\cite{nguyen2015join, aberger2017emptyheaded, sun2020rapidmatch}.
The graph data is organized with several tables as demonstrated in the following example:

\begin{example}
	\label{exp-simple-graph}
	For a data graph with the topological structure demonstrated as $G$ in Fig.\ref{fig-pattern-graph-example} with homogeneous edges,
	Fig.\ref{fig-relation}(b) shows a typical table that stores all edges for relation-based graph data processing. 
	Each edge is stored as a quadruple: $\langle srcId, dstId, eId, label\rangle$, where: \emph{srcId} and \emph{dstId} for the id of the \emph{src} and \emph{dst} vertex respectively; \emph{eId} and \emph{label} for the \emph{id} and \emph{label} of the edge.
\end{example}

\eat{show (1) why the locality cannot be considered, (2) the implicate connection between tuples requires a costly join (3) inefficient for deep queries and travelling.
	
	\textcolor{red}{(there are several optimization strategises for the 
		conventional relational database but the model itself prevents it to achieve a comprehensive optimization)}
}
Processing graph data directly inside the existing RDBMS can therefore gain supports from the various physical design strategies that have been developed so far, as the partition with clustered index demonstrated in Fig.\ref{fig-relation}(c). 
However, such a kind of supports are relatively restricted, the number of the partitions is typically limited while the traversal through different tuples still requires to access the index for the costly \emph{join} operation.
Therefore, they are mainly considered for distributed database instead of providing a more compact memory layout for cache performance improvement.

Excepts the most simplified one above, the relation-based graph data processing system can also be used to describe more complicated graph data:

\eat{
	\textcolor{blue}{The number of partition are typically limited and can bring overhead if it is too many}
	\textcolor{blue}{(SQL server: The database engine supports up to 15,000 partitions by default. In versions earlier than SQL Server 2012 (11.x), the number of partitions was limited to 1,000 by default.)}
	\textcolor{blue}{(MySQL: Beginning with MySQL 5.6.7, this limit is increased to 8192 partitions)}
}


\begin{example}
	\label{exp-heter-graph}
	With the same topological structure of $G$ in Fig.\ref{fig-pattern-graph-example}, 
	both the \emph{vertices} and \emph{edges} in the data graph held in Fig.\ref{fig-relation}(d) are heterogeneous: 
	$v_0,v_2$ have \emph{label} only; 
	$v_1,v_3$ have \emph{attr}  only; 
	$edges_{0 \sim 3}$ have \emph{label} only; 
	and $edges_{4 \sim 5}$ have both \emph{label} and \emph{attr}.
	Both the \emph{vertices/edges} would therefore be stored in separated tables, even the \emph{edges} connect to the same vertex.
	
	Meanwhile, in this case,
	the additional \emph{joins} between the table of $vertex$ and $edge$ would be required for the traversal to access the information on $vertex$
	as shown in Fig.\ref{fig-relation}(d), which would make the query execution process more costly.
\end{example}

\eat{
\etitle{Polyglot data management}. 
The \emph{variety} of big data~\cite{russom2011big, sagiroglu2013big, buhl2013big, laney20013d} 
brings a strong need of \emph{polyglot data management}~\cite{kiehn2022polyglot, khine2019review} for 
the practitioners to handle data with different models in separated stores~\cite{gupta2016cross, tan2017enabling, levy1996querying, halevy2006data, golshan2017data}.
	
Such a deep query is only possible when there are specified consideration for data organization for the \emph{joins} it involves.

In RDBMS, the model for data to be described in SQL and for logic organization are basically the same.
Both in SQL it would be regarded as relation and the data would also be organizes as tables logically, and allow the same value to be joined together. 
In physical level, however, various detailed physical design can be considered, that not necessary requires them to be organized as row-store.

In GDBMS, with basically the same expressiveness of RA, the querying languages on graph typically represent the computing with patterns and sometime the access on property of \emph{vertex/edge}~\cite{francis2018cypher}.
Meanwhile, the logical model for graph data organization provides detailed restrictions for physical design, instead of providing various detail physical design.

\etitle{First order logic}.

\begin{example}
\label{exp-relational-algebra}
The following relational query with natural join:
\begin{align*}
	f \Join  g
\end{align*}
on the database in Fig.\ref{fig-relation}(a),
is equivalent to the first-order-logic query:
\begin{align*}
	\forall x,\forall y,\forall z, f(x,y) \land g(x,z)
\end{align*}
interpreted by Fig.\ref{fig-relation}(a).
\end{example}

Excepts the \emph{relational model} that can consider all possible implicit \emph{``relationship-between-entities''} with the \emph{relational algebra}, \emph{graph} is another widely utilized model that focuses on specified few of them:
}
}
\vspace{-0.4ex}



==> sec-sql-extension.tex <==
\vspace{-0.3ex}
%%%%%%%% Section 1 %%%%%%%%

\section{Hybrid Query with SQL Extension}
\label{sec-sql-extension}

\eat{%%EAT
In this section, a mild extension of the SQL is first provided for users to query across the relational and graph data,
which can also consider the semantic connections between the entities.
}

We first introduce \SQLd, a dialect of \SQL to express
\SQL queries, graph pattern queries \reviseC{and} hybrid queries. %and \emph{``resolution-aware query''}. 


\vspace{-0.3ex}
\etitle{Preliminaries}. A database schema is specified
as $\R = (R_1, \ldots, R_m)$,
where each $R_i$ is a relation schema with a fixed set of attributes.
A tuple $t$ of $R_i$ consists of values, one for each attribute of $R_i$. 
A relation of $R_i$ is a set of tuples of $R_i$. 
A database $\D$ of $\R$ is $(D_1, \ldots, D_m)$, where $D_i$ is
a relation of $R_i$ for $i \in [1, m]$ (see~\cite{abiteboul1995foundations} for 
details).
Following Codd~\cite{codd1979extending},
we assume  that each tuple $t$ represents an entity.\looseness=-1

\eat{Define the label of the vertices/edges in graph as an attribute with special name.
Meanwhile, there are suppose to be attribute, otherwise it would be impossible for entity resolution.}

\begin{figure}[t]
	\vspace{-1.4ex}
	\centerline{\includegraphics[scale=1.9]{./fig/fig-relation.eps}}
	\centering
	\vspace{-2.4ex}
	\caption{
		(a) Database as an interpretation of predicates. 
		(b) A relational representation of homogeneous data graph. 
		(c) An illustration of clustered index and data partition strategies.
		(d) A relational representation for heterogeneous data graph.}
	\label{fig-relation}
	\vspace{-3ex}
\end{figure}


\etitle{Graphs}. A {\em graph}, \warn{label or unlabel(?)}, is specified as $G = (V, E,
\reviseC{L}, F_A)$, where
(a) $V$ is a finite set of vertices;
(b) $E \subseteq V \times V$ is a finite set of edges,
in which $(v, v')$ denotes an edge
from vertex $v$ to $v'$;
(c) \reviseC{function $L$ assigns a label $L(v)$ (resp. $L(e)$) to each $v \in V$ (resp. $e \in E$)};
%Here an edge label typifies predicates while vertex labels carry values.
%Graph $G$ can be directed or undirected.
and (c) \reviseC{each vertex} $v \in V$ (resp.~ edge $e \in E$)
carries a tuple $F_A(v) = (A_1 = a_1,...,A_n = a_n)$ 
(resp.~$F_A(e) = (B_1 = b_1, \ldots , B_m = b_m)$)
of {\em attributes} of a finite arity, written as $v.A_i = a_i$ 
(resp. $e.B_i = b_i$), and $A_i \neq A_j$ (resp. $B_i \neq B_j$)
if $i \neq j$.
%\revise{There are attributes on both vertices and edges.}

We assume the existence of a special attribute \id at each vertex
$v$, denoting its vertex identity, 
such that for any two vertices $v$ and
$v'$ in $G$, if $v.\id = v'.\id$, 
then $v$ and $v'$ refer to the same entity.

\vspace{0.3ex}
\reviseC{Note that the attributes are defined on both
vertices and edges, hence vertex labels $L(v)$ and edge labels
$L(e)$ can
also be uniformly regarded as attributes with special names.}
\warn{Define a special attribute key for label, to suppot both with or without label?}

\looseness=-1 

\eat{%%EAT 
The \emph{``label''} of vertex (resp.~edge) would 
therefore be regarded as an attribute with a special name.
\looseness=-1
}


\etitle{Patterns}. A {\em graph pattern} is defined as
$P = (V_P, E_P, L_P)$, where
$V_P$ (resp.~$E_P$) is a set
of pattern vertices (resp.~pattern edges) and
$L_P$ is a labeling function as above.
\looseness=-1


\eat{Considering topological structure only in the pattern matching.}
\looseness=-1

\etitle{Matches}. A {\em match of a  pattern $P $ in
a graph $G$} is a homomorphic mapping
$h$ %V_P \cup E_P \shortrightarrow V \cup E$, s.t.
from $V_P$ to $V$ such that (a) for each pattern 
vertex $u \in V_P$, $L_P(u) = L(h(u))$; and
(b) for each pattern edge $e = (u, u') \in E_P$, 
there is an edge $(h(u), h(u'))$ in graph $G$ labeled $L_P(e)$.
\warn{According  to the current definition, the edges would be distinguished in the matching.}

\eat{Collect all attributes of vertex and edge to a relation.}
\looseness=-1

\etitle{Pattern queries}. A {\em graph pattern query} is 
$P[\bar A]$, where (a) $P$ is a graph pattern, and (b)
$\bar A$ is a list of attributes such that each $A_i$ in $\bar A$
is attached to a pattern vertex or edge in $P$;
in particular, $A_0$ is an \id attribute attached to
a designated vertex in $P$, \ie entity of interest.  

We represent the {\em result} $P[\bar A](G)$
of a graph pattern query $P[\bar A]$
over graph $G$ as a relation $S$ of schema $R_P$ that is composed
of the attributes $\bar A$. Specifically,
each match $h$ of $P$ in $G$ is encoded
as a tuple $s$ in relation $S$,
such that for each $A_i$ in $\bar A$ that is attached to
pattern vertex $u$ (resp. edge $e$), $s.A_i = h(u).A_i$
(resp. $s.A_i = h(e).A_i$). Here $h(e)$ refers to the
edge in $G$ matching $e$.

\eat{%%EAT
Given a pattern $P = (V_P, E_P)$, data graph $G = (V, E, F_A)$
and a set of attributes 
$\bar A = \{A_{V_{i,j}}\} \cup \{A_{E_{i,j}}\}$ 
of both vertices and edges.
A \emph{graph pattern query} $P[\bar A](G)$ is a relation $R_P$, 
where each match $h: V_P \cup E_P \shortrightarrow V \cup E$ from $P$ to $G$ would extract
a tuple $\bar b = \{b_{V_{i,j}}\} \cup \{b_{E_{i,j}}\} \in R_P$ from $G$,
where $B_{V_{i,j}} = b_{V_{i,j}} \in F_A(h(v_i))$ for $v_i \in V_P$
and $B_{E_{i,j}} = b_{E_{i,j}} \in F_A(h(e_i))$ for $e_i \in E_P$.



\revise{
	Graph pattern matching has been considered as one of the core functionalities for querying graphs~\cite{barcel2011querying, barcel2013querying, davoudian2018survey, peter2012query, angles2017foundations, angles2018GCORE, angles2012comparison, angles2018property, hogan2021knowledge, alin2022Graph},
	which is enabled as a feature in most of the graph query languages~\cite{sparql, sparql11, TinkerPop, francis2018cypher, pienta2016VISAGE, huahai2008graphs,rest2016PGQL,ma2016g,TigerGraph,openCypher},
	and is supported by numerous 
	GDBMS~\cite{allegrogaph, DEX, Filament, GStore, Infinitegraph, SonesGraphDB, vertexdb, neo4j, iordanov2010HyperGraphDB, TinkerPop, TigerGraph}.
	Pattern queries  are becoming increasing ubiquitous:
	$16/60$ of literatures in~\cite{hegeman2018survey},
	$32/40$ of practitioners in~\cite{angles2018GCORE},
	$14/36$ of researchers and
	$19/53$ of practitioners in~\cite{SahuMSLO2020ubiquity}
	concentrate on graph pattern matching.
	They are also adopted in a wide-range of real world applications,
	across biology~\cite{koyuturk2004efficient, li2005interaction, royer2008unraveling},
	security~\cite{jiang2010identifying}, 
	software engineering~\cite{cheng2009identifying, eichinger2008mining, liu2006gplag, maxwell2010diagnosing, surian2010mining, zimmermann2008predicting}, chemistry~\cite{nijssen2004frequent, wegner2006data} and others~\cite{FraudDetect}.
}
}

\eat{%%EAT
Holding a same assumption, we also assume the users can manage to extract a corresponding 
relation from graph where each tuple represents an entity in it,
by writing a correct pattern based on their knowledge of the graph structure.
}

\vspace{0.3ex}
Intuitively, besides topological matching,
the pattern queries also
extract important properties $\bar A$ for entities of interests
(vertices) from the data graphs. These are organized in the 
form of relations.

\eat{
We denote by $P[\bar A](G)$ the set of all attributes $\bar A$
extracted from all matches of
pattern $P$ in graph $G$, which is a relation of the schema
$R_P$ of $P$.}


\stitle{RA$_\delta$}. We now present a dialect of relational algebra
(\RA), denoted by \RAd. A query of \RAd has one of the following forms:
\vspace{-0.7ex}
\beqnn
Q &::=& R\ |\ \pi_{\bar A} Q\ |\ \sigma_C Q\ |\ Q_1 \join Q_2\ |\
Q_1 \cup Q_2\ |\ Q_1 \setminus Q_2 \ |\ \\
&&  P[\bar A](G) \ |\ Q_1 \join_\delta Q_2.
\eeqnn

\vspace{-0.7ex}

\noindent
Here  (a) $R, \pi, \sigma, \join, \cup $ and $\setminus$ denote
relation atom, projection, selection, (natural) join, union
and set difference, respectively, just like their counterpart
in the classic \RA (see~\cite{abiteboul1995foundations}); 
(b) $P[\bar A](G)$ is a {\em graph pattern query} as defined above;
it returns a relation of schema $R_P$, where $G$ is (the name of)
a graph; 
and (c) 
$Q_1 \join_\delta Q_2$ ``joins''
two %relations 
queries, either relational queries or graph pattern queries,
based on their semantic connection, referred to as a 
{\em $\delta$-join}.
\looseness=-1

\etitle{The semantics of $\delta$-join}.
Suppose that $Q_1$ is
a relational query $Q$ and 
$Q_2$ is a graph pattern query $P[\bar A]$; 
the cases for joining queries of the same type are similar.
Assume that over a database $\D$ of schema
$\R$, sub-query $Q(\D)$ returns a relation $D$ of schema
$R_Q$ with attributes $\bar B$; and over graph $G$,
$P[\bar A](G)$ returns a relation $S$ of schema $R_P$.
%with attributes $\bar A$. 



The $\delta$-join $Q \join_\delta P[\bar A](G)$ works as
follows: 
%(1) $S$ would be constructed as an \revise{extended relation, would be defined in Section~~\ref{subsec-define-model},} from $G$ with pattern matching; 
for each tuple $t \in D$ and each tuple $s \in S$,
if $t$ and (vertex) $s$ 
refer to the same real-world
entity, then it returns tuple $t$ 
augmented with attributes in $s$.
The schema of the result of the $\delta$ join can be readily
deduced from $R_Q$ and $R_P$, \ie combining
attributes $\bar A$ and $\bar B$.


\vspace{0.3ex}
Intuitively, for each tuple  $t$ dynamically computed
by query $Q(\D)$, 
this $\delta$-join locates entities $s$ that are
identified by $P[\bar A](G)$ 
and semantically refer to the same entity
as $t$; it extracts properties of $s$ and 
incorporates them into $t$
as additional attributes.
Graph pattern 
matching~\cite{dave2016graphframes, angles2018GCORE,
alin2022Graph, francis2018cypher}
and entity resolution~\cite{TriQL, agrawal2009trio, altwaijry2015query, bhattacharya2006query, 
sismanis2009resolution} are combined here to 
query across \warn{relational and graph data,
or graph and graph data as in~\cite{francis2018cypher}}.


\eat{%%EAT
, two kinds of SQL extensions:
\emph{``graph pattern matching sub-language''}~\cite{dave2016graphframes, angles2018GCORE, alin2022Graph, francis2018cypher} and 
\emph{``resolution-aware query''}~\cite{TriQL, agrawal2009trio, altwaijry2015query, bhattacharya2006query, sismanis2009resolution},
are combined together here to query across relational and graph data from difference sources.

It also works the same to join two graphs together, both directly and semantically, 
	as the feature introduced in Cypher-10~\cite{francis2018cypher}.
}


\begin{example}
\label{exa-join}
\warn{Following Example~\ref{exa-running}, give queries for
	(a) enriching relations and (b) pattern queries with
	relational predicates; justify why the results are
	more meaningful than, \eg $Q \join P[\bar A](G)$}
\end{example}

Several methods %for \emph{``query-aware resolution''} 
are already in place 
to %support \emph{``resolution-aware query''}
integrate entity resolution in query processing, %would 
which determine whether two tuples refer to the same 
entity during query time
with additional operator:
the ETJ/Lineage in~\cite{TriQL, agrawal2009trio};
polymorphic operators in~\cite{altwaijry2015query};
hyper-edge in~\cite{bhattacharya2006query};
entity aggregation with \emph{``Mapping''} in~\cite{sismanis2009resolution}. 
\SystemName \warn{ integrate JedAI~\cite{papadakis2020three}}
inside \RDBMS to support $\delta$-join (Section~\ref{sec-hybrid-query-evaluation}).

\stitle{SQL$_\delta$}. We next present \SQLd. Over database
schema $\R = (R_1, \ldots, R_n)$ and graph $G$, an \SQLd query
has the form:

\vspace{-0.3ex}
\mat{1.0ex}{
	\SELECT\ \ \= $A_{1}$, \ldots, $A_{h}$\\
	\FROM\> $R_{1}$,  \ldots,  $R_{n}$,\\
	\> $P_1[\bar A_1](G)$,\ \ldots,\ $P_k[\bar A_k](G)$, \\
	\> $S_{1}\ \kw{join}\ P_1'[\bar A_1'](G)$,\ \ldots,\
	   $S_{m}\ \kw{join}\ P_m'[\bar A_m'](G)$\\
	%   \warn{$G$ $g_1$, \ldots, $G$ $g_k$} \\
	\WHERE\> {\sc Condition-1} \{\And|\Or\} %{\sc  Condition-2}
	\ldots \{\And|\Or\}  {\sc  Condition-p}
}
\vspace{-0.4ex}

\noindent
Here $S_{1}$, \ldots, $S_{m}$ are either relations in $\R$ or \SQLd
sub-queries over $\R$ and $G$.
An \SQLd query may embed a normal \SQL query,
a pattern query $P_i[\bar A_i](G)$,
and a $\delta$-join $S_{j}\ \kw{join}\ P_j'[\bar A_j'](G)$. 
Each {\sc Condition} in the \WHERE clause is
an \SQL condition over relations $R_{1}$, \ldots, $R_{n}$,
and the result relations of pattern queries and $\delta$-joins.

%Equivalently as a intuitive interface, 
Following~\cite{dave2016graphframes, angles2018GCORE, alin2022Graph, francis2018cypher},
``ASCII-art'' style path is adopted here for 
users to describe the patterns.

\eat{
\textbf{
	Define the \SQLd extension by combining the~\cite{szarnyas2018incremental, szarnyas2018reducing, marton2017formalising}
	and the~\cite{agrawal2009trio,altwaijry2015query,bhattacharya2006query,sismanis2009resolution}
}
}



\begin{example}
	\label{exa-SQL}
	\warn{Write \RAd queries of Example~\ref{exa-join}
		in \SQLd} \revise{(to match with Example~\ref{exa-running})}
\eat{\smaller[1.5]
\begin{lstlisting}[
	language=SQL,
	showspaces=false,
	basicstyle=\linespread{0.8}\ttfamily,
	commentstyle=\color{gray}
	]
      SELECT 
        T.attr0, T.attr1, G.attr2
      FROM (
        SELECT
          attr0, attr1, attr2
        FROM relation ) AS T
      <@\textbf{\textcolor{red}{MAP}}@> ( 
        SELECT
          a.attr0, b.attr1, c.attr2
        FROM graph
        <@\texttt{\textbf{\textcolor{red}{MATCH}}}@>
          (a: A) -[W]-> (    ) -[X]-> (b: B)
        <@\textbf{\textcolor{red}{MATCH}}@>
          (a: A) -[Y]-> (c: C) -[Z]-> (b: B) 
        WHERE a.id != b.id AND a.id != c.id ) AS G;
\end{lstlisting}
With the \textcolor{red}{MAP} to enable the \emph{``resolution-aware query''} as in~\cite{TriQL,agrawal2009trio,altwaijry2015query,bhattacharya2006query,sismanis2009resolution},
and the \textcolor{red}{MATCH} to enable the pattern-based query on graph as in~\cite{ma2016g, angles2018GCORE, alin2022Graph, zhao2019sql, andries1996hybrid, hassan2018grfusion, hassan2017empowering}, 
the extension of SQL here can therefore address the \emph{variety} of big data as required in Example~\ref{exa-join}.
}
\end{example}

%Meanwhile, as would be shown 
As will be seen in Section~\ref{sec-hybrid-query-evaluation}, all \SQLd queries can be
evaluated inside \RDBMS along the same lines as \SQL
queries, without switching to another system
or invoking expensive graph operators.

\eat{
	It would be demonstrated in Section~\ref{subsec-hybrid-query-mapping} how such a query can be mapped on the \emph{relational view} 
	provided in Section~\ref{subsec-relational-view}.
	After that, 
	Section~\ref{sec-hybrid-query} would discuss how the proposed \tbf model can provide an unified plan space to query across relational and graph data, for an in-depth fusion to support more efficient execution, 
	as well as how the query on the \emph{relational view} can be rewritten to execute on the \tbf model data.
	
	Section~\ref{subsec-semantic-hybrid-query-execution} would discuss how the \emph{relational view} can be constructed for semantic hybrid query,
	to avoid the overhead for data extraction as in [\textcolor{red}{SemanticJoin}].
	
	It is unrealistic for a fine definition of the SQL extension, as in \cite{jindal2014graphiql, rest2016PGQL, angles2018GCORE, alin2022Graph}, to be given especially within at most one section here.
	The idea of language-level extension for graph-relation hybrid query itself is not new and cannot be regarded as a core-contribution.
	The limited space should be utilized to provide several examples to demonstrate how semantic query works.
}



\vspace{-0.4ex}

